SybilFence: Improving Social-Graph-Based Sybil Defenses with User Negative Feedback

Detecting and suspending fake accounts (Sybils) in online social networking (OSN) services protects both OSN operators and OSN users from illegal exploitation. Existing social-graph-based defense schemes effectively bound the accepted Sybils to the total number of social connections between Sybils and non-Sybil users. However, Sybils may still evade the defenses by soliciting many social connections to real users. We propose SybilFence, a system that improves over social-graph-based Sybil defenses to further thwart Sybils. SybilFence is based on the observation that even well-maintained fake accounts inevitably receive a significant number of user negative feedback, such as the rejections to their friend requests. Our key idea is to discount the social edges on users that have received negative feedback, thereby limiting the impact of Sybils' social edges. The preliminary simulation results show that our proposal is more resilient to attacks where fake accounts continuously solicit social connections over time.

==> system-overview.tex <==
\section{system overview}
\label{sec:overview}

\subsection{System and threat model}

We model the underlying social graph as a undirected graph $G^+ = (V, E^+)$, where $V$ is the user set in 
the OSN, and $E^+$ represents the social relationships among users. The social relationships represent
friendships or communication relationships in OSNs. On the other hand, we model the network of negative 
feedback as a directed graph $G^- = (V, E^-)$, where $V$ is the same user set as in $G^+$, $E^-$ is the 
direct edge set that includes the negative feedbacks between users. The negative feedback comprises of user 
rejection to friendship requests, user report of abusive communications, machine-learning-based negative  
signal that is generated on behalf of users in response to abusive and harmful communications, etc. Given a 
direction between each pair of users, we consider no more than one negative feedback edge. 
%We do not consider duplicated negative feedback along the same direction of a pair of users.
Figure~\ref{fig:system_model} shows both the social graph and the negative feedback graph sharing the same 
user set in an OSN. In such an OSN, there are $n = |V|$ users, $m = |E^+|$ undirected social edges, 
$k = |E^-|$ directed negative feedback edges, and a node $v$ has a degree of $deg^+(v)$ in $G^+$ and an 
in-degree of $deg^-(v)$ in $G^-$.

\begin{figure}[t!]
\begin{center}
\epsfig{file=figures/system_model.eps, height=4.0cm}
\caption{\bf \footnotesize The social graph and the negative feedback graph in an OSN. 
\label{fig:system_model}}
\end{center}
\end{figure}

In our threat model, malicious users launch Sybil attacks by creating many fake accounts. We divide the 
user set $V$ into two disjoint subsets: non-Sybil users and Sybils, as shown in 
Figure~\ref{fig:system_model}. We denote the 
{\it non-Sybil region} as the collection of the non-Sybil users, and the social relationships and negative 
feedbacks among them. Similarly, the {\it Sybil region} is the collection of the non-Sybil users, and the 
inter-Sybil social relationships and negative feedbacks. We refer to the social relationships between the 
non-Sybil region and the Sybil region as {\it attack edges}. We refer to the Sybils adjacent to the attack 
edges as {\it entrance Sybils}. Entrance Sybils infiltrate the non-Sybil region by 
flooding friendship requests to non-Sybil users, and exploit the resulting friendships by sending unwanted 
communication such as spam through them. As a result, although well-maintained Sybils may be able to 
establish many attack edges to the non-Sybil region, they also receive negative feedback in response from 
cautious non-Sybil users, such as rejection to friendship requests or report of abuse.


\subsection{Assumptions}

We make the following assumptions on the social graph and the negative feedback graph.

\paragraph{Social graph.}
The part of the social graph in the non-Sybil region is well connected and non-bipartite.
This ensures that existing social-graph-based Sybil defenses such as SybilRank~\cite{Cao-NSDI-12} and
SybilLimit~\cite{Yu-SP-08} accept most of non-Sybil users.

\paragraph{Negative feedback graph.}
Users in OSN generate negative feedback in response to abusive communication, such as flooding 
friendship requests and spam messages. A subset of machine-learning techniques can be used to
signal negative feedback on behalf of the receiver of the abusive communication if the receiver
is unaware. The negative feedback can only be triggered by unwanted invitation, abusive activities or communications,
which makes it non-manipulable(\S\ref{}). We assume the negative feedback from users or the selected
machine-learning techniques are trustworthy.

\paragraph{Attack edges and negative feedbacks between the Sybil region and non-Sybil region.}
We relax the prior assumption in social-graph-based Sybil defenses~\cite{Cao-NSDI-12, Yu-SP-08}: 
Sybils always get limited attack edges to non-Sybil users. This assumption may not always hold if
the Sybils are well maintained to keep soliciting social links. Instead, we assume that the Sybils
may be able to obtain many social links to real users, but the attack edges come along with 
negative feedbacks from cautious users. On the other hand, real users only occasionally arouse 
negative feedback due to some mistakes.



\subsection{Goals}

\sys aims to improve the detection accuracy of social-graph-based Sybil defenses using the negative
feedback that accompanies Sybils' abusive activities and communications. In principle, \sys is able
to detect the Sybils collectives that manage to obtain many attack edges to real users, but at the 
same time have annoyed them.

